Learning Intersections of Two Margin Halfspaces under Factorizable Distributions

Learning intersections of halfspaces is a central problem in Computational Learning Theory. Even for just two halfspaces, it remains a major open question whether learning is possible in polynomial time with respect to the margin $\gamma$ of the data points and their dimensionality $d$. The best-known algorithms run in quasi-polynomial time $d^{O(\log(1/\gamma))}$, and it has been shown that this complexity is unavoidable for any algorithm relying solely on correlational statistical queries (CSQ). In this work, we introduce a novel algorithm that provably circumvents the CSQ hardness barrier. Our approach applies to a broad class of distributions satisfying a natural, previously studied, factorizability assumption. Factorizable distributions lie between distribution-specific and distribution-free settings, and significantly extend previously known tractable cases. Under these distributions, we show that CSQ-based methods still require quasipolynomial time even for weakly learning, whereas our algorithm achieves $poly(d,1/\gamma)$ time by leveraging more general statistical queries (SQ), establishing a strong separation between CSQ and SQ for this simple realizable PAC learning problem. Our result is grounded in a rigorous analysis utilizing a novel duality framework that characterizes the moment tensor structure induced by the marginal distributions. Building on these structural insights, we propose new, efficient learning algorithms. These algorithms combine a refined variant of Jennrich's Algorithm with PCA over random projections of the moment tensor, along with a gradient-descent-based non-convex optimization framework.

==> prelim.tex <==
%!TEX root = main.tex


\section*{Appendix} 


\section{Preliminaries and Notations}\label{sec notation}
In this section, we present a complete list of notations, preliminaries and related background on the statistical learning model.


\paragraph{Basic Notations}
In this paper, we use small boldface characters for vectors. For $n \in \Z_+$, we denote by $[n]:=\{1,\dots,n\}$. For $\bx \in \R^d$, and $i \in [d]$, we use $\bx_i$ to denote the $i$-coordinate of $\bx$. For $i \in [d]$, we denote by $\be_i$ the $i$-th standard basis of $\R^d$.
Let $V \subseteq \R^d$ be a subspace, we denote by $\bx_V: = \proj_V (\bx_V)$, the projection of $\bx_V$ onto the subspace $V$ and denote by $V^\perp$ the orthogonal complement of $V.$ For $\bu,\bv \in \R^d$, we use $\bu \cdot \bv$ to denote the inner product of $\bu$ and $\bv$ and we use $\norm{\bu}_2$ to denote the $\ell_2$ norm of $\bu$. We use $S^{d-1}=\{\bx\in\R^n:\|\bx\|_2=1\}$ to denote the $d$-dimensional unit sphere.


For any distribution $D$, we use $\E_{\bx\sim D}(\bx)$ to denote the expectation of $D$. Let $D$ be a distribution of $(\bx,y)$ over $\R^d \times \{\pm 1\}$. We use $D_X$ to denote the marginal distribution of $D$ over $\R^d$.
For any subspace $V \subseteq \R^d$, we use $D_V$ to denote the marginal distribution of $D$ for $\bx_V$. For $z \in \{\pm 1\}$, we use $D^z_V$ to denote the marginal distribution of $D$ over $\bx_V$ condition on $y=z$ and use $D^z$ to denote the marginal distribution $D_X$ over $\bx$ condition on $y=z$
For a distribution $D_X$ over $\R^d$, we say $D_X$ has an isotropic covariance matrix if there is some $\alpha\ge 0$ such that $\E_{\bx \sim D_X}\bx\bx^\intercal = \alpha I$, where $\alpha$ is called the scale of $\E_{\bx \sim D_X}\bx\bx^\intercal$.


For tensors, 
we will consider a $k$-tensor to be an element in $(\mathbb{R}^n)^{\otimes k}\cong\mathbb{R}^{n^k}$.
A symmetric tensor is a tensor that is invariant under a permutation of its vector arguments. We use $\norm{T}_F$ to denote the Frobinius norm of $T$.
We will use $T_{i_1,\ldots,i_k}$ to denote the coordinate of a $k$-tensor $T$ indexed by the $k$-tuple $(i_1,\ldots,i_k)$. 
By abuse of notation, we will sometimes also use this to denote the entire tensor.
The inner product of a $k$-tensor is defined by thinking of the tensor as a vector with $n^k$ coordinates
and then using the definition of the inner product of vectors.
For a vector $\bv\in\R^n$, we denote by $\bv^{\otimes k}$ to be a vector (linear object) in $\R^{n^k}$.
For a matrix $M\in\R^{n\times m}$, we denote by $\|M\|_2,\|M\|_F$ to be the operator norm and Frobenius norm respectively.
%In addition, we denote by $M^{\otimes k}$ to be a matrix (linear operator) mapping $\R^{n^k}$ to $\R^{m^k}$.

\new{
By abuse of notation,
we will sometimes treat a tensor $T\in (\R^d)^{\otimes m}$ as a linear mapping, i.e., for $\bv\in \R^d$, we use $T\bv$ to denote applying the linear mapping $T:\R^d\to (\R^d)^{\otimes m-1}$ specified by $T$ on $\bv$.

}


\begin{fact} \label{fct:lb-tensor-random-rank1-correlation}
    Let $T\in (\R^d)^{\otimes m}$ and $\|T\|_F=1$ be a symmetric tensor for $m\leq 3$, then $\max_{\bu\in S^{d-1}} \bu^{\otimes m}\cdot T\geq 1/\poly(d)$.
\end{fact}

%\mnote{define sym in the appendix}

\begin{proof}
    For a tensor $T\in (\R^d)^{\otimes m}$ and $\pi:[m]\to [m]$ be a permutation of indices,
    we use $\pi(T)$ to denote the tensor permuted by $\pi$ defined as 
    $\pi(T)_{\pi(i_1),\cdots,\pi(i_m)}=T_{i_1,\cdots,i_m}$.
    We define $\sym(T)$ as $\frac{1}{m!}\sum_{\pi\in \Pi}\pi(T)$, where $\Pi$ is the set of all possible permutations of $[m]$.
    
    The statement trivially holds for $m=1,2$. Therefore, we only need to consider the case $m=3$. 
    We first show that any symmetric $T\in (\R^d)^{\otimes 3}$ can be written as 
    $
    T=\sum_{i=1}^N \alpha_i \bv_i^{\otimes 3}\; ,
    $
    where $N=\poly(d)$ and $\sum_{i=1}^N |\alpha_i|=\poly(d)$.
    Suppose we have shown that this is true, then it is easy to see that 
    $1= T\cdot T =\sum_{i=1}^N \alpha_i {\bv_i}^{3}\cdot T\leq \poly(d)\max_i ( {\bv_i}^{3}\cdot T)$, therefore at least one $\bv_i$ satisfies ${\bv_i}^{3}\cdot T=1/\poly(d)$.
    
    Therefore, we just need to show that the statement above about decomposition is true.
    Since $\sym(\bv_i\otimes \bv_j\otimes \bv_k)$ where $\bv_i, \bv_j,\bv_k$ are standard basis vectors span the space of symmetric tensors.
    Therefore, it suffices for us to show that the statement holds true for any such $\sym(\bv_i\otimes \bv_j\otimes \bv_k)$.
    Notice that 
    \[(\bv_i+\bv_j)^{\otimes 3}-\bv_i^{\otimes 3}-\bv_i^{\otimes 3}=3\sym(\bv_i\otimes \bv_j^{\otimes 2})+3\sym(\bv_j\otimes \bv_k^{\otimes 2})\; , \] and
    \[(\bv_i-\bv_j)^{\otimes 3}-\bv_i^{\otimes 3}+\bv_i^{\otimes 3}=3\sym(\bv_i\otimes \bv_j^{\otimes 2})-3\sym(\bv_j\otimes \bv_k^{\otimes 2})\; . \]
    This shows that the decomposition statement is true for any $\sym(\bv_i\otimes \bv_j^{\otimes 2})$.
    Then, using $\sym(\bv_i\otimes \bv_j^{\otimes 2})$ notice that 
    \[
    \sym(\bv_i\otimes (\bv_j+\bv_k)^{\otimes2})-\sym(\bv_i\otimes \bv_j^{\otimes 2})-\sym(\bv_i\otimes \bv_k^{\otimes 2})=2\sym(\bv_i\otimes \bv_j\otimes \bv_k)\; .
    \]
    This completes the proof.
\end{proof} 




%\mnote{Also need to add SQ model}


\paragraph{Background on Statistical Query Model}
SQ algorithms are a class of algorithms that are allowed
to query expectations of bounded functions on the underlying distribution 
through an (SQ) oracle
rather than directly access
samples. The model was introduced by \cite{Kearns:98} as a natural restriction of the PAC 
model~\citep{Valiant:84} in the context of learning Boolean functions. 
Since then, the SQ model has been extensively studied in a range of settings, including
unsupervised learning~\citep{Feldman16b}.
The class of SQ algorithms is broad and captures a range of known 
algorithmic techniques in machine learning including spectral techniques,
moment and tensor methods, local search (e.g., EM),
and many others (see, e.g.,~\cite{FeldmanGRVX17, FeldmanGV17} 
and references therein).

\begin{definition}[SQ Model] \label{def:sq}
Let $D$ be a distribution on $X$. 
A \emph{statistical query} is a bounded function $q:X\rightarrow[-1,1]$. 
We define $\mathrm{STAT}(\tau)$ to be the oracle that given any such query $q$, outputs a value $v$ such that $|v-\E_{x\sim D}[q(x)]|\leq\tau$, where $\tau>0$ is the \emph{tolerance} parameter of the query.
A \emph{statistical query (SQ) algorithm} is an algorithm 
whose objective is to learn some information about an unknown 
distribution $D$ by making adaptive calls to the corresponding $\mathrm{STAT}(\tau)$ oracle.
\end{definition}

%In particular, given $D$ is a distribution on $X\times \{\pm 1\}$, we can define the Correlational Statistical Query (CSQ) model as a further restriction of the SQ model. In the CSQ model, the query function $q:X\times \{\pm 1\}\to [-1,1]$ is required to always satisfy $q(x,1)=-q(x,-1)$ for any $x\in X$.

\paragraph{Basics of Correlational Statistical Query(CSQ) Model}

In particular, given $D$ is a distribution on $X\times \{-1, 1\}$, we can define the Correlational Statistical Query (CSQ) model as a further restriction of the SQ model. 

\begin{definition} [CSQ Model] \label{def:csq}
Let $D$ be a distribution on $X\times \{-1,1\}$. 
A \emph{correlational statistical query} is a bounded function $q:X\times \{-1,1\}\rightarrow[-1,1]$. 
We define $\mathrm{CSTAT}(\tau)$ to be the oracle that given any such query $q$, outputs a value $v\in [-1,1]$ such that $|v-\E_{(\bx,y)\sim D}[yq(\bx)]|\leq\tau$, where $\tau>0$ is the \emph{tolerance} parameter of the query.
A \emph{statistical query (SQ) algorithm} is an algorithm 
whose objective is to learn some information about an unknown 
distribution $D$ by making adaptive calls to the corresponding $\mathrm{STAT}(\tau)$ oracle. 
\end{definition}

\begin{definition} [Function Representation of Distribution for CSQ]
Let $D$ be a joint distribution of $(\bx,y)$ supported on $\R^d\times \{\pm 1\}$ where $D^+$ and $D^-$ has probability density functions $P_{D^+}, P_{D^-}:\R^d\to \R_+$.
Let $D_0$ be a distribution on $\R^d$ with density function $P_{D_0}:\R^d\to \R+$ where the support of $D$ contains the support of $D^+$ and $D^-$.
Then, the function representation of $D$ for CSQ w.r.t. $D_0$ is defined as a function $f_D:\R^d\to \R$ such that $f_D(\bx)=(P_{D^+}(\bx)-P_{D^-}(\bx))/P_{D_0}(\bx)$.
\end{definition}

\begin{definition} [Pairwise Correlation]
For functions $f,g:\R^d\mapsto \R_+$, we defined the correlation between $f$ and $g$ under the distribution $D_0$ to be the expectation 
$\E_{\bx\sim D_0}[f(\bx)g(\bx)]$.
\end{definition}

\begin{definition}
We say that a set of functions $F$ mapping $\R^d\to \R$ is 
$(\gamma,\beta)$-correlated relative to a distribution $D$ if for any $f_i,f_j\in F$,
the correlation $\E_{\bx\sim D_0}[f_i(\bx)f_j(\bx)]\leq  \gamma$ for all $i\neq j$
and $\E_{\bx\sim D_0}[f_i(\bx)f_j(\bx)]\leq  \beta$ for $i=j$.
\end{definition}






\begin{definition} [Decision Problem over Distributions] \label{def:decision-problem}
Let $D$ be a fixed distribution and $\cal D$ be a distribution family. 
We denote by $\mathcal{B}(\D,D)$ the decision problem in which 
the input distribution $D'$ is promised to satisfy either (a) $D'=D$ or (b) $D'\in \D$,
and the goal is to distinguish the two cases with high probability.
\end{definition}





\begin{definition} [Correlational Statistical Query Dimension]
For $\beta,\gamma>0$, a decision problem $\mathcal{B}(\D,D_0)$, where $D_0$ is a fixed distribution and 
$\D$ is a family of distribution, let $s$ be the maximum integer such that
there exists a finite set of distributions $\D_D\subseteq\D$ such that 
$\{f_{D'}-f_{D}\mid D'\in \D_D\}$ is $(\gamma,\beta)$-correlated relative to $D$ and $|\D_D|\geq s$. 
The Correlational Statistical Query dimension with pairwise correlations $(\gamma,\beta)$ of $\mathcal{B}$ is defined to be $s$, 
and denoted by $s=\mathrm{CD}(\mathcal{B},\gamma,\beta)$.
\end{definition}

\begin{lemma}\label{lem:sq-lb}
Let $\mathcal{B}(\D,D)$ be a decision problem, where $D$ is 
the reference distribution and $\D$ is a class of distribution. For $\gamma,\beta>0$, 
let $s=\mathrm{CD}(\mathcal{B},\gamma,\beta)$. 
For any $\gamma'>0$, any CSQ algorithm for $\mathcal{B}$ requires queries of tolerance 
at most $\sqrt{\gamma+\gamma'}$ or makes at least $s\gamma'/(\beta-\gamma)$ queries.
\end{lemma}








% \begin{enumerate}
%     \item vector, inner product, projection, (finished)
%     \item distribution, expectation, $D^+,D^-$ (finished)
%     \item tensor operation, tensor norm, matrix norm (checked)
%     \item SQ, CSQ
%     \item tensor lemma
%     \item LP related 
%     \item polynomial 
%     We will construct a polynomial $p(\bx)=\sum_{i,j,k\in \{0,1\}^3,i\leq j\leq k}a_{i,j,k}\bx_{i}\bx_{j}\bx_{k}$. For choosing the value of parameter $a$.
    
% \end{enumerate}


% We will use lowercase boldface letters for vectors and capitalized boldface letters for matrices and tensors.
% We use $\mathbb{S}^{n-1}=\{\bx\in\R^n:\|\bx\|_2=1\}$ to denote the $n$-dimensional unit sphere.
% For vectors $\bu,\bv\in\R^n$, we use $\langle\bu,\bv\rangle$ to denote the standard inner product.
% For $\bu\in \R^n$, we use $\|\bu\|_k=\big (\sum_{i=1}^n \bu_i^k\big )^{1/k} $ to denote the $\ell_k$-norm of $\bu$.
% For tensors, 
% we will consider a $k$-tensor to be an element in $(\mathbb{R}^n)^{\otimes k}\cong\mathbb{R}^{n^k}$.
% This can be thought of as a vector with $n^k$ coordinates.
% We will use $A_{i_1,\ldots,i_k}$ to denote the coordinate of a $k$-tensor $A$ indexed by the $k$-tuple $(i_1,\ldots,i_k)$. 
% By abuse of notation, we will sometimes also use this to denote the entire tensor.
% The inner product and $\ell^k$-norm of a $k$-tensor are defined by thinking of the tensor as a vector with $n^k$ coordinates
% and then using the definition of inner product and $\ell_k$-norm of vectors.
% For a vector $\bv\in\R^n$, we denote by $\bv^{\otimes k}$ to be a vector (linear object) in $\R^{n^k}$.
% For a matrix $\bV\in\R^{n\times m}$, we denote by $\|\bV\|_2,\|\bV\|_F$ to be the operator norm and Frobenius norm respectively.
% In addition, we denote by $\bV^{\otimes k}$ to be a matrix (linear operator) mapping $\R^{n^k}$ to $\R^{m^k}$.



% 1. tensor operation: $T_k$ denotes a tensor operation for $k$ times 2. tensor norm

% We define the following decision problem over distributions.








